Quantum Public-Key Encryption with Tamper-Resilient Public Keys from One-Way Functions

We construct quantum public-key encryption from one-way functions. In our construction, public keys are quantum, but ciphertexts are classical. Quantum public-key encryption from one-way functions (or weaker primitives such as pseudorandom function-like states) are also proposed in some recent works [Morimae-Yamakawa, eprint:2022/1336; Coladangelo, eprint:2023/282; Barooti-Grilo-Malavolta-Sattath-Vu-Walter, eprint:2023/877]. However, they have a huge drawback: they are secure only when quantum public keys can be transmitted to the sender (who runs the encryption algorithm) without being tampered with by the adversary, which seems to require unsatisfactory physical setup assumptions such as secure quantum channels. Our construction is free from such a drawback: it guarantees the secrecy of the encrypted messages even if we assume only unauthenticated quantum channels. Thus, the encryption is done with adversarially tampered quantum public keys. Our construction is the first quantum public-key encryption that achieves the goal of classical public-key encryption, namely, to establish secure communication over insecure channels, based only on one-way functions. Moreover, we show a generic compiler to upgrade security against chosen plaintext attacks (CPA security) into security against chosen ciphertext attacks (CCA security) only using one-way functions. As a result, we obtain CCA secure quantum public-key encryption based only on one-way functions.

==> construction_old.tex <==
% !TEX root = main.tex
\section{Construction of QPKE}
\label{sec:construction}
In this section, we construct a QPKE scheme that satisfies correctness and IND-pkTA security (but not decryption error detectability) from PRFs and digital signatures. 
The message space of our construction is $\bit$, but it can be extended to be arbitrarily many bits by parallel repetition. 
Let $\{\PRF_k:\bit^u\to\bit^n\}_{k\in \bit^\secp}$ be a quantum-query secure PRF and $(\Gen,\Sign,\Ver)$ be an EUF-CMA secure digital signature scheme with a deterministic $\Sign$ algorithm.
%We assume that the verification key of the digital signature scheme is already sent to
%the sender in an authenticated way. Moreover, the signing key of the digital signature scheme is
%possessed by the receiver. (These assumptions are also made implicitly in classical PKE.)

Our construction of QPKE is as follows.
\begin{itemize}
    \item 
    $\SKGen(1^\secp)\to(\sk,\vk):$
    Choose $k_0,k_1\gets\bit^\secp$.
    Run $(\mathsf{sigk},\vk)\gets\Gen(1^\secp)$.
    Output $\sk\coloneqq(k_0,k_1,\mathsf{sigk})$ and $\vk$. 
    \ryo{This is a minor syntactical issue. $\vk$ is used as a verification key of QPKE. However, in the signature key pair, $\vk$ is used as a verification of signature. It is better to use a different notation for the signature vefication key (say, $\sfsig.\vk$ and set $\vk \seteq \sfsig.\vk$).}\takashi{I'm fine with using $\vk$ to mean both because this is somewhat obvious.}
    \item
    $\PKGen(\sk)\to\pk:$
    Parse $\sk=(k_0,k_1,\mathsf{sigk})$.
    Choose $r\gets\bit^u$.
    By running $\PRF$ and $\Sign$ coherently, generate a state $\ket{\psi_0}+\ket{\psi_1}$ over registers $(\regA,\regB,\regC)$,
    where
    \begin{align}
    \ket{\psi_0}&\coloneqq \ket{0}_\regA\otimes\ket{\PRF_{k_0}(r)}_\regB\otimes\ket{\sigma(r\|0\|\PRF_{k_0}(r))}_\regC,\\
    \ket{\psi_1}&\coloneqq \ket{1}_\regA\otimes\ket{\PRF_{k_1}(r)}_\regB\otimes\ket{\sigma(r\|1\|\PRF_{k_1}(r))}_\regC.
    \end{align}
    Here $\sigma(\alpha)\coloneqq\Sign(\mathsf{sigk},\alpha)$ is the signature for the message $\alpha$.
    (For simplicity, we omit $\mathsf{sigk}$.)
    Output 
    \begin{align}
    \pk&\coloneqq(r,\ket{\psi_0}+\ket{\psi_1}).
    \end{align}
   \item
   $\Enc(\vk,\pk,b)\to\ct:$
   Parse
    $\pk=(r,\rho)$, where $\rho$ is a quantum state over registers $(\regA,\regB,\regC)$. 
    The $\Enc$ algorithm consists of the following three steps. 
   \begin{enumerate}
    \item
    It coherently checks the signature in $\rho$. In other words, it applies the unitary
   \begin{equation}
      U_{r,\vk}\ket{\alpha}_\regA\ket{\beta}_\regB\ket{\gamma}_\regC\ket{0...0}_\regD
      =\ket{\alpha}_\regA\ket{\beta}_\regB\ket{\gamma}_\regC\ket{\Ver(\vk,r\|\alpha\|\beta,\gamma)}_\regD
   \end{equation} 
    on $\rho_{\regA,\regB,\regC}\otimes|0...0\rangle\langle0...0|_\regD$, and
    measures the register $\regD$ in the computational basis. If the result is $\bot$, it outputs $\ct\coloneqq\bot$ and halts.
    If the result is $\top$, 
    it goes to the next step.
    \item
    It applies $Z^b$ on the register $\regA$. 
    \item
    It measures all qubits in the Hadamard basis to get the result $d$.
    It outputs
    \begin{equation}
    \ct\coloneqq(r,d).
    \end{equation}
    \end{enumerate}
   \item
   $\Dec(\sk,\ct)\to b':$
   Parse $\sk=(k_0,k_1,\mathsf{sigk})$ and
    $\ct=(r,d)$.
    Output 
    \begin{equation}
    b'\coloneqq d\cdot 
    (0\|\PRF_{k_0}(r)\|\sigma(r\|0\|\PRF_{k_0}(r))
    \oplus 1\|\PRF_{k_1}(r)\|\sigma(r\|1\|\PRF_{k_1}(r))).
    \end{equation}
\end{itemize}

The correctness is straightforward. 
First, the state over the register $(\regA,\regB,\regC)$ is
$\ket{\psi_0}+\ket{\psi_1}$ if $\pk$ was not tampered with and the first step of $\Enc$ algorithm got $\top$.
Second, in that case, the state becomes $\ket{\psi_0}+(-1)^b\ket{\psi_1}$ after the second step of $\Enc$ algorithm.
Finally, because in that case $d$ obtained in the third step of $\Enc$ algorithm satisfies
    \begin{equation}
    b=d\cdot 
    (0\|\PRF_{k_0}(r)\|\sigma(r\|0\|\PRF_{k_0}(r))
    \oplus 1\|\PRF_{k_1}(r)\|\sigma(r\|1\|\PRF_{k_1}(r))),
    \end{equation}
    we have $b'=b$.


==> pure_old.tex <==
% !TEX root = main.tex
\section{Pure State Public Key Variant}\label{sec:pure_pk_qpke}
As discussed in \Cref{sec:discussion}, we believe that the distinction between pure state and mixed state public keys is not important from a practical point of view. Nonetheless, it is a mathematically valid question if we can construct an IND-pkTA secure QPKE scheme with pure state public keys. We give such a scheme based on the existence of subexponentially secure OWFs 
%quantum-secure OWFs 
by extending the construction given in \Cref{sec:construction}. 

\subsection{Preparation}
We state the definition of subexponentially secure OWFs for clarity.
\begin{definition}
    A subexponentially secure OWF is a function $f:\bit^* \rightarrow \bit^*$ that satisfies the following for some0 constant $c>0$: For any quantum adversary $\cA$ that runs in time $2^{c\secp}$, 
    \begin{equation}
        \Pr[f(x')=f(x):x\gets \bit^\secp,x' \gets \A(1^\secp, f(x))]\le 2^{-c\secp}.
    \end{equation}
\end{definition}
\begin{remark}
    Subexponentially secure OWFs sometimes only require the one-wayness advantage (the LHS in the above inequality) to be inverse-subexponential for all \emph{QPT} adversaries. Our definition is stronger than that since we require  the one-wayness advantage to be inverse-subexponential for all \emph{subexponentual-time} adversaries.
\end{remark}

We introduce a fine-grained version of strong EUF-CMA security. 
\begin{definition}[$\epsilon$-strong EUF-CMA security]
A digital signature scheme $(\Gen,\Sign,\Ver)$ is $(T,\epsilon)$-strong EUF-CMA secure if the following holds: 
For any quantum adversary $\cA$ that runs in time $T$ and makes at most $T$ classical queries to the signing oracle $\Sign(k,\cdot)$,
\begin{equation}
   \Pr[(\msg^\ast,\sigma^\ast)\notin \mathcal{Q}~\land~\top\gets\Ver(\vk,\msg^*,\sigma^*):
   (k,\vk)\gets\Gen(1^\secp),
   (\msg^\ast,\sigma^\ast)\gets\cA^{\Sign(k,\cdot)}(\vk)
   ]\le \epsilon, 
\end{equation}
where $\mathcal{Q}$ is the set of message-signature pairs returned by the signing oracle. 
\end{definition}
By applying a standard complexity leveraging argument to the proof of \Cref{thm:sig_from_OWF} in \cite[Sec. 6.5.2]{Book:Goldreich04}, one can show the following:
\begin{theorem}\label{thm:sig_from_OWF_subexp}
For any constant $c>0$, there exist 
$(2^{c\secp},2^{-c \secp})$-strong EUF-CMA secure digital signatures if subexponentially secure OWFs exist.
\end{theorem}

\iffalse
We define quantum-query pseudorandom functions which are used in our construction. 
\begin{definition}[Pseudorandom functions (PRFs)]
A keyed function $\{\PRF_K: \cX\rightarrow \cY\}_{K\in \bit^\secp}$ that is computable in classical deterministic polynomial-time is a quantum-query secure pseudorandom function if 
for any QPT adversary $\cA$ with quantum access to the evaluation oracle $\PRF_K(\cdot)$,
\begin{equation}
   |\Pr[1\gets\cA^{\PRF_K(\cdot)}(1^\secp)] 
   -\Pr[1\gets\cA^{H(\cdot)}(1^\secp)] |\le\negl(\secp),
\end{equation}
where $K\gets\bit^\secp$ and $H:\cX\rightarrow \cY$ is a function chosen uniformly at random.
\end{definition}
\begin{remark}
Quantum-query secure PRFs exist if quantum-secure OWFs exist~\cite{FOCS:Zhandry12}.
\end{remark}

We also need the following lemma in the security proof.
\begin{lemma}\label{lem:cannot_find_both}
For a function $H:\bit^{u+1}\rightarrow \bit^v$, let $\ket{\psi_H}:=\sum_{R\in \bit^{u+1}}\ket{R}\ket{H(R)}$. For any integer $m$ and (unbounded-time) quantum algorithm $\A$, 

\begin{align}
    \Pr_{H}[
    y_0=H(0\concat r)~\land~y_1=H(1\concat r)
    :(r,y_0,y_1)\gets \A(\ket{\psi_H}^{\otimes m})]\le (2m+1)^4(2^{-u}+2^{-v})
\end{align}
where $H$ is a uniformly random function from $\bit^{u+1}$ to $\bit^v$. 
\end{lemma}

This can be proven by using the result of \cite{EC:YamZha21}. We defer the proof to \Cref{sec:proof_lemma}.
\fi

\subsection{Construction}
In this section, we construct a QPKE scheme that satisfies correctness and IND-pkTA security (but not decryption error detectability) and has pure state public keys from 
$T$-strong EUF-CMA secure digital signatures for exponential $T$. %and quantum-query secure PRFs. 
The message space of our construction is $\bit$, but it can be extended to be arbitrarily many bits by parallel repetition. 
Let $(\Gen,\Sign,\Ver)$ be a $(2^{2u},2^{-2u})$-strong EUF-CMA secure digital signature scheme with a deterministic $\Sign$ algorithm and message space $\bit^u$  %$\bit^{u+v+1}$,   
%and $\{\PRF_K:\bit^{u+1} \rightarrow \bit^v\}_{K\in \bit^\secp}$ be a quantum-query secure PRF 
where $u=\omega(\log \secp)$. %and $v=\omega(\log \secp)$.  
Note that such a digital signature scheme exists assuming the existence of subexponentially secure OWFs by \Cref{thm:sig_from_OWF_subexp}.
%We assume that the verification key of the digital signature scheme is already sent to
%the sender in an authenticated way. Moreover, the signing key of the digital signature scheme is
%possessed by the receiver. (These assumptions are also made implicitly in classical PKE.)

Our construction of QPKE is as follows.
\begin{itemize}
    \item 
    $\SKGen(1^\secp)\to(\sk,\vk):$
    Run $(k,\vk)\gets\Gen(1^\secp)$.
    Output $\sk\seteq k$. Output $\vk$.  
    %$\SKGen(1^\secp)\to(\sk,\vk):$ Run $(k,\vk)\gets\Gen(1^\secp)$ and sample $K\gets \bit^\secp$. Output $\sk\coloneqq (k,K)$ and $\vk$. 
    \item
    $\PKGen(\sk)\to\pk:$
    Parse $\sk=k$.
    By running $\Sign$ coherently, generate the state
    \begin{align}
    \ket{\psi_\sk}\seteq\sum_{r\in \bit^u}\ket{r}_{\regR}\otimes \left(\ket{0}_\regA\otimes\ket{\Sign(k,0\|r)}_\regB
    +\ket{1}_\regA\otimes\ket{\Sign(k,1\|r)}_\regB\right)
    \end{align}
    over registers $(\regR,\regA,\regB)$.
    Output 
    \begin{align}
    \pk&\seteq \ket{\psi_\sk}.
    \end{align}
    %$\PKGen(\sk)\to\pk:$
    %Parse $\sk=k$.
    %Parse $\sk=(k,K)$.
    %Choose $r\gets\bit^u$.
    %By running $\Sign$ and $\PRF$ coherently, generate the state 
    %\begin{eqnarray}
    %\ket{\psi_\sk}\coloneqq
    %\sum_{r\in \bit^u}\ket{r}_{\regR}\otimes 
   % \left( 
  %  \begin{array}{l}
%\ket{0}_\regA\otimes\ket{y(0,r)}_\regB \otimes \ket{\sigma(0,r)}_\regC\\
 %   +\ket{1}_\regA\otimes\ket{y(1,r)}_\regB \otimes \ket{\sigma(1,r)}_\regC
    %  \end{array}
    %\right)
    %\end{eqnarray} 
    %over registers $(\regR,\regA,\regB,\regC)$
    %where 
    %$y(b,r):=\PRF_K(b\concat r)$
    %and
    %$\sigma(b,r):=\Sign(k,b\concat r\concat y(b,r))$
    %for $b\in \bit$ and $r\in \bit^u$. (We omit $K$ and $k$ from the notations for simplicity.)
    %Output 
    %\begin{align}
    %\pk&\coloneqq\ket{\psi_\sk}.
    %\end{align}
   \item
   $\Enc(\vk,\pk,b)\to\ct:$
   Parse
    $\pk=\rho$, where $\rho$ is a quantum state over registers $(\regR,\regA,\regB)$. %$(\regR,\regA,\regB,\regC)$. 
    The $\Enc$ algorithm consists of the following three steps. 
   \begin{enumerate}
    \item
    It coherently checks the signature in $\rho$. In other words, it applies the unitary
   \begin{equation}
      U_{\vk}\ket{r}_{\regR}\ket{\alpha}_\regA\ket{\beta}_{\regB}\ket{0...0}_\regD
      =\ket{r}_{\regR}\ket{\alpha}_\regA\ket{\beta}_{\regB}\ket{\Ver(\vk,\alpha\|r,\beta)}_\regD
   \end{equation} 
    on $\rho_{\regR,\regA,\regB}\otimes|0...0\rangle\langle0...0|_\regD$, and
    measures the register $\regD$ in the computational basis. 
   %\begin{equation}
   %   U_{\vk}\ket{r}_{\regR}\ket{\alpha}_\regA\ket{\beta}_{\regB}\ket{\gamma}_\regC\ket{0...0}_\regE
   %   =\ket{r}_{\regR}\ket{\alpha}_\regA\ket{\beta}_{\regB}\ket{\gamma}_\regC\ket{\Ver(\vk,\alpha\|r\|\beta,\gamma)}_\regE
   %\end{equation} 
    %on $\rho_{\regR,\regA,\regB,\regC}\otimes|0...0\rangle\langle0...0|_\regE$, and measures the register $\regE$ in the computational basis. 
    If the result is $\bot$, it outputs $\ct\coloneqq\bot$ and halts.
    If the result is $\top$, 
    it goes to the next step.
    \item
    It applies $Z^b$ on the register $\regA$. 
    \item
    It measures 
    $\regR$ in the computational basis to get $r$ and 
    all qubits in the registers $(\regA,\regB)$  %$(\regA,\regB,\regC)$ 
    in the Hadamard basis to get the result $d$.
    It outputs
    \begin{equation}
    \ct\coloneqq(r,d).
    \end{equation}
    \end{enumerate}
   \item
   $\Dec(\sk,\ct)\to b':$
   Parse $\sk=(k,K)$ and
    $\ct=(r,d)$.
    Output 
    \begin{equation}
    b'\coloneqq d\cdot 
    (0\|\Sign(k,0\|r) \oplus 1\|\Sign(k,1\|r))
    %(0\|y(0,r)\|\sigma(0,r) \oplus 1\|y(1,r)\|\sigma(1,r)).
    \end{equation}
\end{itemize}

\begin{theorem}\label{thm:IND-pkTA_QPKE_from_SIG_pure}
If $(\Gen,\Sign,\Ver)$ is a $(2^{2u},2^{-2u})$-strong EUF-CMA secure digital signature scheme %and $\{\PRF_K:\bit^{u+1} \rightarrow \bit^v\}_{K\in \bit^\secp}$ be a quantum-query secure PRF, 
then the QPKE scheme $(\SKGen,\PKGen,\Enc,\Dec)$ above is correct and IND-pkTA secure.
\end{theorem}
\begin{proof}[Proof (sketch)]
The correctness is easily seen similarly to the proof of \Cref{thm:IND-pkTA_QPKE_from_SIG}. 

For IND-pkTA security, we only explain the differences from the proof of \Cref{thm:IND-pkTA_QPKE_from_SIG} since it is very similar. We define Hybrid $0,1$, and $2$ similarly to those in the proof of \Cref{thm:IND-pkTA_QPKE_from_SIG}. For clarity, we describe them in \cref{hyb0_pure,hyb1_pure,hyb2_pure}. 

Assume that the IND-pkTA security of our construction is broken by a QPT adversary
$\cA$. It means the QPT adversary $\cA$ wins Hybrid 0 with a non-negligible advantage.
Then, it is clear that there is another QPT adversary $\cA'$ that wins Hybrid 1  
with a non-negligible advantage. ($\cA'$ has only to do the Hadamard-basis measurement by itself.)

From the $\cA'$, we construct a QPT adversary $\cA''$ that wins 
Hybrid 2 with a non-negligible probability based on a similar proof to that in   \cref{sec:B}. 
Indeed, the proof is almost identical once we show a counterpart of \cref{why}. For proving the counterpart of \cref{why}, we use $(2^{2u},2^{-2u})$-strong EUF-CMA security of the digital signature scheme. The crux of the original proof of \cref{why} is that the adversary given polynomially many public keys can output a valid signature for a message that is not of the form $b\|\Sign(k,b\|r)$ only with a negligible probability.  This can be easily reduced to strong EUF-CMA security in the mixed state public key case since the adversary does not obtain superposition of signatures over messages containing different $r$'s. On the other hand, due to the modification of the public key, the adversary now has polynomially many copies of 
$\ket{\psi_\sk}$
    which involves all $r$'s in superposition.
For proving that the adversary given polynomially many copies of the above public key can output a valid signature for a message that is not of the form $b\|\Sign(k,b\|r)$ only with a negligible probability, we consider a reduction algorithm that queries signatures on \emph{all} $b\|r$ for $b\in \bit$ and $r\in \bit^u$. 
Thus, the reduction algorithm makes $2^{u+1}$ and runs in time $2^u\cdot \poly(\secp)$. Since we have $2^{u+1}<2^{2u}$ and $2^u\cdot \poly(\secp)<2^{2u}$ for sufficiently large $\secp$, the above reduction enables us to prove the above property assuming the $(2^{2u},2^{-2u})$-strong EUF-CMA security of the digital signature scheme.

Thus, it suffices to prove that no adversary can win Hybrid 2 with a non-negligible probability.  This can be done similarly to the proof in \Cref{sec:Zhandry}, but there is a difference that we need to guess the $r$ used in the challenge ciphertext, which cases an exponential security loss. Let Hybrid 3 be the same as Hybrid 2 except that a uniformly random $r^\ast$ is chosen at the beginning and aborts if $r\neq r^\ast$ (see \Cref{hyb3_pure}).  
Then, we have 
\begin{align}
\Pr[\cA~\text{wins Hybrid~}3]= 2^{-u}\cdot \Pr[\cA~\text{wins Hybrid~}2].
\end{align}
On the other hand, by a similar argument to that in \Cref{sec:Zhandry}, we can show 
\begin{align}
\Pr[\cA~\text{wins Hybrid~}3]\le 2^{-2u+1}
\end{align}
by the $(2^{2u},2^{-2u})$-strong EUF-CMA security and \Cref{lem:BZ}
where the reduction algorithm queries signatures on all messages of the form $b\|r$ for $b\in \bit$ and $r\neq r^{\ast}$ and either of $0\|r^\ast$ or $1\|r^\ast$. \takashi{I may add more explanation.}
Thus, 
\begin{align}
\Pr[\cA~\text{wins Hybrid~}2]\le 2^{-u+1}=\negl(\secp).
\end{align}
This completes the proof of \Cref{thm:IND-pkTA_QPKE_from_SIG_pure}.  
%By almost the same argument as in the proof of \Cref{thm:IND-pkTA_QPKE_from_SIG} using the strong EUF-CMA security of the digital signature scheme, IND-pkTA security is reduced to that the adversary's winning probability is negligible in Hybrid 2 in \Cref{hyb_pure} for any QPT algorithm $\A$ and polynomial $m$.\footnote{We call it Hybrid 2 for consistency to the proof in \Cref{sec:security}.} 

\protocol{Hybrid 0}
{Hybrid 0}
{hyb0_pure}
{
\begin{enumerate}
%    \item 
%    The challenger $\cC$ chooses $k_0,k_1\gets\bit^\secp$.
    \item \label{item:initial_pure}
    $\cC$ runs $(k,\vk)\gets\Gen(1^\secp)$.
    $\cC$ sends $\vk$ to $\cA$.
  \item
    $\cC$ sends $\ket{\psi_{\sk}}^{\otimes m}$
    to the adversary $\cA$, where
   \begin{align}
    \ket{\psi_\sk}\seteq\sum_{r\in \bit^u}\ket{r}\otimes \left(\ket{0}\otimes\ket{\Sign(k,0\|r)}
    +\ket{1}\otimes\ket{\Sign(k,1\|r)}\right)
    \end{align}
    \item
    \label{Ar_pure}
    $\cA$ generates a quantum state over registers $(\regR,\regA,\regB,\regC)$. 
    ($(\regR,\regA,\regB)$ corresponds to the quantum part of $\pk'$, and $\regC$ corresponds to $\st$.)
    $\cA$ sends the registers $(\regR,\regA,\regB)$ to $\cC$.
    $\cA$ keeps the register $\regC$.
    \item
    \label{sign_pure}
    $\cC$ coherently checks the signature in the state sent from $\cA$.
    If the result is $\bot$, it sends $\bot$ to $\cA$ and halts.
    If the result is $\top$, it goes to the next step. 
   
    \item
    \label{bchosen_pure}
    $\cC$ chooses $b\gets \bit$.
    $\cC$ applies $Z^b$ on the register $\regA$.
 \item
    $\cC$ measures $\regR$ in the computational basis to get $r$. 
    \item
    $\cC$ measures all qubits in $(\regA,\regB)$ in the Hadamard basis to get the result $d$.
    $\cC$ sends $(r,d)$ to $\cA$.
    \item
    \label{last_pure}
    $\cA$ outputs $b'$.
    If $b'=b$, $\cA$ wins.
\end{enumerate}
}


\protocol{Hybrid 1}
{Hybrid 1}
{hyb1_pure}
{
\begin{itemize}
    \item[1.-6.]
    All the same as \cref{hyb0_pure}.
    \item[7.]
    $\cC$ does not do the Hadamard-basis measurement,
    and $\cC$ sends $r$ and registers $(\regA,\regB)$ to $\cA$.
    \item[8.]
    The same as \cref{hyb0_pure}.
\end{itemize}
}


\protocol{Hybrid 2}
{Hybrid 2}
{hyb2_pure}
{
\begin{itemize}
    \item[1.-7.]
    All the same as \cref{hyb1_pure}.
    \item[8.]
    $\cA$ outputs $(\mu_0,\mu_1)$.
    If $\mu_0=\Sign(k,0\|r)$ and $\mu_1=\Sign(k,1\|r)$, $\cA$ wins.
\end{itemize}
}

\protocol{Hybrid 3}
{Hybrid 3}
{hyb3_pure}
{
\begin{itemize}
    \item[0.] $\cC$ chooses $r^\ast\gets \bit^u$. 
    \item[1.-8.]
    All the same as \cref{hyb2_pure} except that $\cA$ loses if $r\neq r^\ast$. 
\end{itemize}
}

\iffalse
\protocol{Hybrid 2}
{Hybrid 2}
{hyb_pure}
{
\begin{enumerate}
%    \item 
%    The challenger $\cC$ chooses $k_0,k_1\gets\bit^\secp$.
    \item 
    $\cC$ runs $(k,\vk)\gets\Gen(1^\secp)$ and generates $K\gets \bit^\secp$ and sets $\sk:=(k,K)$.
    $\cC$ sends $\vk$ to $\cA$.
    \item
    $\cC$ sends $\ket{\psi_{\sk}}^{\otimes m}$
    to the adversary $\cA$, where
   \begin{eqnarray}
    \ket{\psi_\sk}\coloneqq
    \sum_{r\in \bit^u}\ket{r}\otimes 
    \left( 
    \begin{array}{l}
\ket{0}\otimes\ket{y(0,r)} \otimes \ket{\sigma(0,r)}\\
    +\ket{1}\otimes\ket{y(1,r)} \otimes \ket{\sigma(1,r)}
      \end{array}
    \right)
    \end{eqnarray} 
     where 
    $y(b,r):=\PRF_K(b\concat r)$
    and
    $\sigma(b,r):=\PRF_K(b\concat r\concat y(b,r))$. 
    \item
    $\cA$ generates a quantum state over registers $(\regR,\regA,\regB,\regC,\regD)$. 
    ($(\regR,\regA,\regB,\regC)$ corresponds to $\pk'$, and $\regD$ corresponds to $\st$.)
    $\cA$ sends the registers $(\regR,\regA,\regB,\regC)$ to $\cC$.
    $\cA$ keeps the register $\regD$.
    \item
    $\cC$ coherently checks the signature in the state sent from $\cA$.
    If the result is $\bot$, it sends $\bot$ to $\cA$ and halts.
    If the result is $\top$, it goes to the next step. 
   
    \item
    $\cC$ applies $Z^{b^\ast}$ on the register $\regA$ for $b^\ast\gets \bit$.

    \item
    $\cC$ measures $\regR$ in the computational basis to get $r$. 
    \item 
    $\cC$  sends $r$ and registers $(\regA,\regB,\regC)$ to $\cA$.
    \item
    $\cA$ outputs $(\mu_0,\mu_1)$.
   $\cA$ wins if $\mu_b=y(b,r)\concat \sigma(b,r)$ for $b\in \bit$. 
\end{enumerate}
}

Let Hybrid 2' be a hybrid that works similarly to Hybrid 2 except that $y(b,r)$ is defined as  $y(b,r):=H(b\concat r)$ for a uniformly random function $H$ instead of $\PRF$. By the quantum-query security of $\PRF$, the winning probabilities in Hybrid 2' and Hybrid 2 are negligibly close. Thus, it suffices to prove the winning probability in Hybrid 2' is negligible. This is proven by a straightforward reduction to \Cref{lem:cannot_find_both} noting that $\ket{\psi_\sk}$ with the modification of $y(b,r)$ as above can be generated from  $\ket{\psi_H}=\sum_{R\in \bit^{u+1}}\ket{R}\ket{H(R)}$ by coherently running $\Sign$. 
This completes the proof of IND-pkTA security.
\fi 
\end{proof}
\begin{remark}
    We can add decryption error detectability by \Cref{thm:add_decryption_error_detectability} and extend it to recyclable QPKE by the construction of \Cref{sec:recyclable}. These extensions preserve the property that public keys are pure states. 
\end{remark}


\iffalse
\subsection{Proof of \Cref{lem:cannot_find_both}}\label{sec:proof_lemma}
For proving \Cref{lem:cannot_find_both}, we rely on the following lemma shown by \cite{EC:YamZha21}. 
\begin{lemma}[{\cite[Theorem 4.2]{EC:YamZha21}}]\label{lem:YZ}
Let $H:\calX\rightarrow \calY$ be a uniformly random function. 
Let $\A$ be an (unbounded-time) randomized algorithm that makes $q$ quantum queries to $H$ and outputs a classical string $z$. 
Let $\mathcal{C}$ be an (unbounded-time) randomized algorithm that takes $z$ as input, 
makes $k$ classical queries to $H$, and outputs $\top$ or $\bot$.
Let $\B$ be the following algorithm that makes at most $k$ classical queries to $H$: 
\begin{description}
\item[$\B^{H}()$:]~ It does the following:
\begin{enumerate}
\item Choose a function $H':\calX\rightarrow \calY$ from a family of $2q$-wise independent hash functions.
    \item 
    For each $j\in[k]$, uniformly pick $(i_j,b_j)\in ([q]\times \bit) \cup \{(\bot,\bot)\}$ under the constraint that there does not exist $j\neq j'$ such that $i_j=i_{j'}\neq \bot$.
    \item Initialize a stateful oracle $\mathcal{O}$ to be a quantumly-accessible classical oracle that computes $H'$.
    \item Run $\A^{\mathcal{O}}()$ where $\mathcal{O}$ is simulated as follows.
   When $\A$ makes its $i$-th query, the oracle is simulated as follows:
    \begin{enumerate}
      \item If $i=i_j$ for some $j\in[k]$, 
        measure $\A$'s  query register to obtain $x'_j$, query $x'_j$ to the random oracle $H$ to obtain $H(x'_j)$, and do either of the following.
        \begin{enumerate}
        \item If $b_j=0$, reprogram 
        $\mathcal{O}$ to output $H(x'_j)$ on $x'_j$ and answer $\A$'s $i_j$-th query by using the reprogrammed oracle. 
        \item If $b_j=1$, answer  $\A$'s $i_j$-th query by using the oracle before the reprogramming and then reprogram 
        $\mathcal{O}$ to output $H(x'_j)$ on $x'_j$. 
        \end{enumerate}
     \item Otherwise, answer $\A$'s $i$-th query by just using the oracle $\mathcal{O}$ without any measurement or  reprogramming.
    \end{enumerate}
    \item Output whatever $\A$ outputs.
\end{enumerate}
\end{description}
Then we have 
\begin{align}
     \Pr_H[\mathcal{C}^H(z)=\top :z\gets \B^{H}()] \geq \frac{1}{(2q+1)^{2k}}\Pr_H[\mathcal{C}^H(z)=\top :z\gets \A^{H}()]. \label{eq:lifting}
\end{align}
\end{lemma}
\begin{remark}
    There are the following  differences  from \cite[Theorem 4.2]{EC:YamZha21} in the statement of the lemma:
    \begin{enumerate}
        \item They consider inputs to $\A$ and $\B$. We omit them because this suffices for our purpose. 
        \item They consider a more general setting where $\A$ and $\B$ interact with $\mathcal{C}$. We focus on the non-interactive setting. 
        \item They do not explicitly write how $\B$ works in the statement of \cite[Theorem 4.2]{EC:YamZha21}. But this is stated at the beginning of its proof. 
    \end{enumerate}
\end{remark}

Using the above lemma, it is easy to prove \Cref{lem:cannot_find_both}.
\begin{proof}[Proof of \Cref{lem:cannot_find_both}]
For an algorithm $\A$ in \Cref{lem:cannot_find_both}, 
let $\tilde{\A}$ be an oracle-aided algorithm that generates $m$ copies of $\ket{\psi_H}$ by making $m$ quantum queries to $H$ on uniform superpositions of inputs and then runs $\A(\ket{\psi_H}^{\otimes m})$. 
Let $\mathcal{C}$ be an oracle-aided algorithm that takes $z=(r,y_0,y_1)$ as input, makes two classical queries $0\|r$ and $1\|r$ to $H$, and outputs $\top$ if and only if $y_0=H(0\concat r)$ and $y_1=H(1\concat r)$.  
By \Cref{lem:YZ}, 
we have 
\begin{align}
     &\Pr_H[ y_0=H(0\concat r)~\land~y_1=H(1\concat r) :(r,y_0,y_1)\gets \tilde{\B}^{H}()]\\ \geq 
     &\frac{1}{(2m+1)^{4}}\Pr_H[ y_0=H(0\concat r)~\land~y_1=H(1\concat r) :(r,y_0,y_1)\gets \tilde{\A}^{H}()] \label{eq:lifting_application}
\end{align}
where $\tilde{\B}$ is to $\tilde{\A}$ as $\B$ (defined in \Cref{lem:YZ}) is to $\A$. 
By the definition of $\tilde{\B}$, it just makes at most two classical queries to $H$ on independently and uniformly random inputs $R_0,R_1$. The probability that we happen to have $\{R_0,R_1\}=\{0\| r,1\|r\}$ for some $r\in \bit^u$ is $2^{-u}$. Unless the above occurs, either  $H(0\concat r)$ or $H(1\concat r)$ is uniformly random to
$\tilde{\B}$ for all $r$, and thus 
the probability that its output satisfies $ y_0=H(0\concat r)$ and $y_1=H(1\concat r)$ is at most $2^{-v}$.
Thus, we have 
\begin{align}
    \Pr_H[ y_0=H(0\concat r)~\land~y_1=H(1\concat r) :(r,y_0,y_1)\gets \tilde{\B}^{H}()]\le 2^{-u}+2^{-v}. \label{eq:upper_bound_tilde_B}
\end{align}
Combining \Cref{eq:lifting_application,eq:upper_bound_tilde_B}, we obtain \Cref{lem:cannot_find_both}. 
\end{proof}
\fi

==> security.tex <==
% !TEX root = main.tex
\section{Proof of IND-pkTA Security}\label{sec:security}
In this section, we show IND-pkTA security of our construction to complete the proof of~\cref{thm:IND-pkTA_QPKE_from_SIG}.
The outline of the proof is as follows.
The security game for the IND-pkTA security of our QPKE (Hybrid 0) is given in \cref{hyb0}.
We introduce two more hybrids, Hybrid 1 (\cref{hyb1}) and Hybrid 2 (\cref{hyb2}).
Hybrid 1 is the same as Hybrid 0 except that the challenger does not do the Hadamard-basis measurement
in the third step of $\Enc$ algorithm, and the challenger sends the adversary $r$ and the state over the registers
$(\regA,\regB)$.
Hybrid 2 is the same as Hybrid 1 except that the adversary outputs two bit strings $\mu_0,\mu_1$ and
the adversary wins if $\mu_0=\Sign(k,0\|r)$ and $\mu_1=\Sign(k,1\|r)$. 
The formal proof is as follows.

Assume that the IND-pkTA security of our construction is broken by a QPT adversary
$\cA$. It means the QPT adversary $\cA$ wins Hybrid 0 with a non-negligible advantage.
Then, it is clear that there is another QPT adversary $\cA'$ that wins Hybrid 1  
with a non-negligible advantage. ($\cA'$ has only to do the Hadamard-basis measurement by itself.)
From the $\cA'$, we can construct a QPT adversary $\cA''$ that wins 
Hybrid 2 with a non-negligible probability 
by using the idea of \cite{HMY22}. (For details, see \cref{sec:B}).
Finally, we show in \cref{sec:Zhandry}
that no QPT adversary can win Hybrid 2 except for a negligible probability.
We thus have the contradiction, and 
therefore our QPKE is IND-pkTA secure.

\protocol{Hybrid 0}
{Hybrid 0}
{hyb0}
{
\begin{enumerate}
%    \item 
%    The challenger $\cC$ chooses $k_0,k_1\gets\bit^\secp$.
    \item \label{item:initial}
    $\cC$ runs $(k,\vk)\gets\Gen(1^\secp)$.
    $\cC$ sends $\vk$ to $\cA$.
    \item
    \label{rs}
    $\cC$ chooses $r_1,...,r_m\gets\bit^u$.
    \item
    \label{send}
    $\cC$ sends $\{(r_i,\ket{\psi_{r_i}})\}_{i=1}^m$
    to the adversary $\cA$, where
    \begin{align}
       \ket{\psi_{r_i}}&\coloneqq
       \ket{0}\otimes\ket{\Sign(k,0\|r_i)}
       +\ket{1}\otimes\ket{\Sign(k,1\|r_i)}.
    \end{align}
    \item
    \label{Ar}
    $\cA$ generates a quantum state over registers $(\regA,\regB,\regC)$. 
    ($(\regA,\regB)$ corresponds to the quantum part of $\pk'$, and $\regC$ corresponds to $\st$.)
    $\cA$ sends a bit string $r$ and the registers $(\regA,\regB)$ to $\cC$.
    $\cA$ keeps the register $\regC$.
    \item
    \label{sign}
    $\cC$ coherently checks the signature in the state sent from $\cA$.
    If the result is $\bot$, it sends $\bot$ to $\cA$ and halts.
    If the result is $\top$, it goes to the next step. 
   
    \item
    \label{bchosen}
    $\cC$ chooses $b\gets \bit$.
    $\cC$ applies $Z^b$ on the register $\regA$.

    \item
    $\cC$ measures all qubits in $(\regA,\regB)$ in the Hadamard basis to get the result $d$.
    $\cC$ sends $(r,d)$ to $\cA$.
    \item
    \label{last}
    $\cA$ outputs $b'$.
    If $b'=b$, $\cA$ wins.
\end{enumerate}
}


\protocol{Hybrid 1}
{Hybrid 1}
{hyb1}
{
\begin{itemize}
    \item[1.-6.]
    All the same as \cref{hyb0}.
    \item[7.]
    $\cC$ does not do the Hadamard-basis measurement,
    and $\cC$ sends $r$ and registers $(\regA,\regB)$ to $\cA$.
    \item[8.]
    The same as \cref{hyb0}.
\end{itemize}
}


\protocol{Hybrid 2}
{Hybrid 2}
{hyb2}
{
\begin{itemize}
    \item[1.-7.]
    All the same as \cref{hyb1}.
    \item[8.]
    $\cA$ outputs $(\mu_0,\mu_1)$.
    If $\mu_0=\Sign(k,0\|r)$ and $\mu_1=\Sign(k,1\|r)$, $\cA$ wins.
\end{itemize}
}








\subsection{From Distinguishing to Outputting Two Signatures}
\label{sec:B}
We present the construction of $\cA''$.
Assume that there exists a QPT adversary
$\cA'$ and a polynomial $p$ such that 
\begin{equation}
|\Pr[1\gets\cA'\mid b=0]-\Pr[1\gets\cA'\mid b=1]|\ge\frac{1}{p(\secp)}
\label{advantage}
\end{equation}
in Hybrid 1 (\cref{hyb1}) for infinitely many $\secp$.
From the $\cA'$, we construct a QPT adversary $\cA''$ such that
\begin{equation}
\Pr[(\Sign(k,0\|r),\Sign(k,1\|r))\gets\cA'']\ge\frac{1}{q(\secp)}
\end{equation}
in Hybrid 2 (\cref{hyb2}) with a polynomial $q$ for infinitely many $\secp$.

Let $t\coloneqq (k,\vk,r_1,...,r_m,r)$, and $\Pr[t]$
be the probability that $t$ is generated in \cref{item:initial}, \cref{rs}, and \cref{Ar} in the game of \cref{hyb1}. 
Let $\mathsf{Good}$ be the event that
$\cC$ gets $\top$ in \cref{sign} in the game of \cref{hyb1}.
Let $\mathsf{Bad}$ be the event that
$\mathsf{Good}$ does not occur.
Then, from \cref{advantage}, we have
\begin{align}
\frac{1}{p(\secp)}&\le
\Big|\sum_t\Pr[t] \Pr[\mathsf{Good} \mid t]\Pr[1\gets\cA' \mid t,\mathsf{Good},b=0]
+\sum_t\Pr[t] \Pr[\mathsf{Bad} \mid t]\Pr[1\gets\cA' \mid t,\mathsf{Bad},b=0]\nonumber\\
&-\sum_t\Pr[t] \Pr[\mathsf{Good} \mid t]\Pr[1\gets\cA' \mid t,\mathsf{Good},b=1]
-\sum_t\Pr[t] \Pr[\mathsf{Bad} \mid t]\Pr[1\gets\cA' \mid t,\mathsf{Bad},b=1]\Big|\\
&\le
\sum_t\Pr[t] \Pr[\mathsf{Good} \mid t]
\Big|\Pr[1\gets\cA' \mid t,\mathsf{Good},b=0]
-\Pr[1\gets\cA' \mid t,\mathsf{Good},b=1]\Big|\nonumber\\
&+\sum_t\Pr[t] \Pr[\mathsf{Bad} \mid t]
\Big|\Pr[1\gets\cA' \mid t,\mathsf{Bad},b=0]
-\Pr[1\gets\cA' \mid t,\mathsf{Bad},b=1]\Big|\\
&=
\sum_t\Pr[t] \Pr[\mathsf{Good} \mid t]
\Big|\Pr[1\gets\cA' \mid t,\mathsf{Good},b=0]
-\Pr[1\gets\cA' \mid t,\mathsf{Good},b=1]\Big|
\end{align}
for infinitely many $\secp$,
because if $\mathsf{Bad}$ occurs, $\cA'$ gets only $\bot$ which contains no information about $b$.
(Here, we often abuse notation to just write $t$ to mean the event that $t$ is generated 
in \cref{item:initial}, \cref{rs}, and \cref{Ar}.)
Therefore, if we define
\begin{equation}
   T\coloneqq\Big\{t:
   \Pr[\mathsf{Good} \mid t]
\cdot \Big|\Pr[1\gets\cA' \mid t,\mathsf{Good},b=0]
-\Pr[1\gets\cA' \mid t,\mathsf{Good},b=1]\Big|\ge\frac{1}{2p(\secp)}
   \Big\}, 
\end{equation}
we have 
\begin{align}
\Pr[\mathsf{Good} \mid t]\ge\frac{1}{4p(\secp)}
\label{goodnonnegl}
\end{align}
and
\begin{align}
\Big|\Pr[1\gets\cA' \mid t,\mathsf{Good},b=0]
-\Pr[1\gets\cA' \mid t,\mathsf{Good},b=1]\Big|
\ge\frac{1}{2p(\secp)}
\label{dif}
\end{align}
for any $t\in T$ and
\begin{align}
\sum_{t\in T}\Pr[t]\ge\frac{1}{2p(\secp)}
\end{align}
for infinitely many $\secp$.


Let $\ket{\phi_b^{t,good}}$ be the state over the registers $(\regA,\regB,\regC)$
immediately before \cref{last} of \cref{hyb1} given that 
$t$ is generated,
$\mathsf{Good}$ occurred,
and $b$ is chosen in \cref{bchosen} of \cref{hyb1}.
We can show the following lemma. (Its proof is given later.)
\begin{lemma}
\label{why}
If $(\Gen,\Sign,\Ver)$ is strong EUF-CMA secure, there exists a subset $T'\subseteq T$ such that $\sum_{t\in T'}\Pr[t]$ is non-negligible
and the following is satisfied (for infinitely many $\secp$):
For any $t\in T'$, $\ket{\phi_b^{t,good}}$ is negligibly close to a state in the form of
    \begin{equation}
    c_0\ket{0}_\regA\ket{\Sign(k,0\|r)}_\regB\ket{\Psi_0}_{\regC}    
    +(-1)^bc_1\ket{1}_\regA\ket{\Sign(k,1\|r)}_\regB\ket{\Psi_1}_{\regC},   
    \label{whystate}
    \end{equation}
    where $c_0$ and $c_1$ are some complex coefficients such that $|c_0|^2+|c_1|^2=1$, 
and $\ket{\Psi_0}$ and $\ket{\Psi_1}$ are some normalized states.
\end{lemma}

Now let us fix $t\in T'$.
Also, assume that $\mathsf{Good}$ occurred.
Because $T'\subseteq T$, it means that $t\in T$.
Then,
from \cref{dif},
\begin{align}
\Big|\Pr[1\gets\cA' \mid t,\mathsf{Good},b=0]
-\Pr[1\gets\cA' \mid t,\mathsf{Good},b=1]\Big|=\Delta
\label{advantage2}
\end{align}
for a non-negligible $\Delta\ge\frac{1}{2p(\secp)}$ for infinitely many $\secp$.
Without loss of generality, we can assume that in \cref{last} of \cref{hyb1},
$\cA'$ applies a unitary $V$ on the state $\ket{\phi_b^{t,good}}$, and
measures the register $\regA$ in the computational basis to get $b'\in\bit$.
By \cref{advantage2}
we have
\begin{align}
V\ket{\phi_0^{t,good}}&=\sqrt{p}\ket{1}_{\regA}\ket{\nu_1}_{\regB,\regC}+\sqrt{1-p}\ket{0}_{\regA}\ket{\nu_0}_{\regB,\regC} \label{eq:V_phi_zero}\\    
V\ket{\phi_1^{t,good}}&=\sqrt{1-p+\Delta}\ket{0}_{\regA}\ket{\xi_0}_{\regB,\regC}+\sqrt{p-\Delta}\ket{1}_{\regA}\ket{\xi_1}_{\regB,\regC}    \label{eq:V_phi_one} 
\end{align}
for some real number $p$ and some normalized states $\ket{\nu_0},\ket{\nu_1},\ket{\xi_0},\ket{\xi_1}$.
(This is because any state can be written as $p\ket{1}\ket{\nu_1}+\sqrt{1-p}\ket{0}\ket{\nu_0}$
with some $p$ and normalized states $\ket{\nu_0},\ket{\nu_1}$, and due to \cref{advantage2}, the coefficients
of $\ket{1}\ket{\xi_1}$ has to be $\sqrt{p-\Delta}$.)
If we define $W$ as
\begin{equation}
   W\coloneqq V^\dagger (Z\otimes I) V, 
\end{equation}
we have
\begin{align}
&   |
   c_0^*c_1\bra{0}\bra{\Sign(k,0\|r)}\bra{\Psi_0}W\ket{1}\ket{\Sign(k,1\|r)}\ket{\Psi_1}\\
   &+c_0c_1^*\bra{1}\bra{\Sign(k,1\|r)}\bra{\Psi_1}W\ket{0}\ket{\Sign(k,0\|r)}\ket{\Psi_0}|\\
  &\simeq\frac{1}{4} |
  (\bra{\phi_0}+\bra{\phi_1})W(\ket{\phi_0}-\ket{\phi_1})
  +(\bra{\phi_0}-\bra{\phi_1})W(\ket{\phi_0}+\ket{\phi_1})
  | \label{eq:rewrite}\\
  &=\frac{1}{2} |
  \bra{\phi_0}W\ket{\phi_0}
  -\bra{\phi_1}W\ket{\phi_1}
  |\\
   \begin{split}
   &=
  \frac{1}{2}\left|\left(\sqrt{p}\bra{1}\bra{\nu_1}+\sqrt{1-p}\bra{0}\bra{\nu_0}\right)
  \left(-\sqrt{p}\ket{1}\ket{\nu_1}+\sqrt{1-p}\ket{0}\ket{\nu_0}\right)\right.\\
  &\left.~~~-
    \left(\sqrt{1-p+\Delta}\bra{0}\bra{\xi_0}+\sqrt{p-\Delta}\bra{1}\bra{\xi_1}\right) 
  \left(\sqrt{1-p+\Delta}\ket{0}\ket{\xi_0}-\sqrt{p-\Delta}\ket{1}\ket{\xi_1}\right)\right|
  \end{split} \label{eq:expand}
  \\
  &=\frac{1}{2}\left|-p+(1-p)-(1-p+\Delta)+(p-\Delta)\right|\\
  & =\Delta 
\end{align}
for infinitely many $\secp$,
where $(t,good)$ of $\ket{\phi_b^{t,good}}$ is omitted for simplicity,
and $\simeq$ means the equivalence except for a negligible difference.
Here, \Cref{eq:rewrite} follows from \cref{why}, and 
\Cref{eq:expand} follows from \Cref{eq:V_phi_zero,eq:V_phi_one} and the definition of $W$. 
From the triangle inequality and the facts that $|c_0|\le1$ and $|c_1|\le1$,
\begin{align}
&\Delta\le
   |c_1|\cdot|\bra{0}\bra{\Sign(k,0\|r)}\bra{\Psi_0}W\ket{1}\ket{\Sign(k,1\|r)}\ket{\Psi_1}|\\
   &+|c_0|\cdot|\bra{1}\bra{\Sign(k,1\|r)}\bra{\Psi_1}W\ket{0}\ket{\Sign(k,0\|r)}\ket{\Psi_0}|
\end{align}
for infinitely many $\secp$.
Then,
\begin{align}
\frac{\Delta}{2}\le
   |c_1|\cdot|\bra{0}\bra{\Sign(k,0\|r)}\bra{\Psi_0}W\ket{1}\ket{\Sign(k,1\|r)}\ket{\Psi_1}|
\end{align}
or
\begin{align}
&\frac{\Delta}{2}\le
  |c_0|\cdot|\bra{1}\bra{\Sign(k,1\|r)}\bra{\Psi_1}W\ket{0}\ket{\Sign(k,0\|r)}\ket{\Psi_0}|
\end{align}
holds for infinitely many $\secp$.
Assume that the latter holds.
(The following proof can be easily modified even if the former holds.)
Then
\begin{align}
\frac{\Delta^2}{4}&\le
   |c_0|^2\cdot|\bra{1}\bra{\Sign(k,1\|r)}\bra{\Psi_1}W\ket{0}\ket{\Sign(k,0\|r)}\ket{\Psi_0}|^2\\
   &\le
   |c_0|^2\cdot\|(I\otimes\bra{\Sign(k,1\|r)}\otimes I)W\ket{0}\ket{\Sign(k,0\|r)}\ket{\Psi_0}\|^2\label{delta}
\end{align}
for infinitely many $\secp$.
With this $W$, we can construct the QPT adversary $\cA''$ that wins the game of \cref{hyb2} with a non-negligible probability as follows.
\begin{enumerate}
    \item 
    Simulate $\cA'$ in steps 1.-7. of \cref{hyb2}. 
    If $\bot$ is sent from $\cC$, output $\bot$ and halt. 
    \item
    Measure the register $\regA$ in the computational basis. If the result is 1, output $\bot$ and halt.
    If the result is 0, measure the register $\regB$ of the post-measurement state in the computational basis to get the measurement result $\mu_0$. 
    \item
    Apply $W$ on the post-measurement state 
    and measure the register $\regB$ in the computational basis to get the result $\mu_1$.
    Output $(\mu_0,\mu_1)$.
\end{enumerate}
Assume that $t\in T'$ and $\mathsf{Good}$ occurred.
Such an event occurs with a non-negligible probability, because
of the following reasons. First,
$\sum_{t\in T'}\Pr[t]$ is non-negligible from \cref{why}.
Second, because $t\in T'$ means $t\in T$, $\Pr[\mathsf{Good} \mid t]$ is non-negligible from
\cref{goodnonnegl}.

From \cref{why}, the state before $\cA''$ measures the register $\regA$ is negligiblly close to
\cref{whystate}.
Then, from \cref{delta},
the probability that $(\mu_0,\mu_1)=(\Sign(k,0\|r),\Sign(k,1\|r))$ is
non-negligible. 

Hence, the overall probability that $\cA''$ outputs $(\mu_0,\mu_1)=(\Sign(k,0\|r),\Sign(k,1\|r))$ is
non-negligible.

We prove~\cref{why} to complete this subsection.
\begin{proof}[Proof of \cref{why}]
Fix $t\in T$.
Immediately before the coherent signature test in \cref{sign} of \cref{hyb1}, the entire state over the registers 
$(\regA,\regB,\regC)$
is generally written as 
\begin{equation}
\sum_{\alpha,\beta}d_{\alpha,\beta}\ket{\alpha}_\regA\ket{\beta}_\regB\ket{\Lambda_{\alpha,\beta}}_{\regC},
\end{equation}
where $d_{\alpha,\beta}$ are some complex coefficients such that $\sum_{\alpha,\beta}|d_{\alpha,\beta}|^2=1$, 
and $\ket{\Lambda_{\alpha,\beta}}$ are some normalized states.
Define the set
\begin{align}
   S\coloneqq\{(\alpha,\beta):\Ver(\vk,\alpha\|r,\beta)=\top\wedge \beta\neq \Sign(k,\alpha\|r)\}. 
\end{align}
The (unnormalized) state after obtaining $\top$ in the coherent signature test in \cref{sign} of \cref{hyb1}
is
\begin{align}
&d_{0,\Sign(k,0\|r)}\ket{0}_\regA\ket{\Sign(k,0\|r)}_\regB
\ket{\Lambda_{0,\Sign(k,0\|r)}}_{\regC}\label{norm1}\\
&+d_{1,\sign(k,1\|r)}\ket{1}_\regA\ket{\Sign(k,1\|r)}_\regB
\ket{\Lambda_{1,\Sign(k,1\|r)}}_{\regC}\label{norm2}\\
&+\sum_{(\alpha,\beta)\in S}d_{\alpha,\beta}\ket{\alpha}_\regA\ket{\beta}_\regB\ket{\Lambda_{\alpha,\beta}}_{\regC}\label{norm3}.
\end{align}

Define 
\begin{equation}
T'\coloneqq\{t\in T:\mbox{the norm of \cref{norm3} is negligible}\}.
\end{equation}
If $\sum_{t\in T'}\Pr[t]$ is negligible,
then $\sum_{t\in T\setminus T'}\Pr[t]$ is non-negligible, but
it contradicts
the strong EUF-CMA security of the digital signature scheme.
Therefore,
$\sum_{t\in T'}\Pr[t]$ is non-negligible.

Moreover, because $t\in T'$ means $t\in T$, $\Pr[\mathsf{Good} \mid t]$ is non-negligible from \cref{goodnonnegl}.
Therefore,
for any $t\in T'$,
the norm of \cref{norm1} plus that of \cref{norm2}
should be non-negligible.
Therefore, 
if we renormalize it and apply $Z^b$, 
the state is negligibly close to
a state in the form of \cref{whystate} (for infinitely many $\secp$).
\end{proof}



\subsection{No QPT Adversary Can Output Two Signatures}
\label{sec:Zhandry}
Here we show that no QPT adversary can win Hybrid 2 (\cref{hyb2}) with a non-negligible probability.
First, note that the probability that all $\{r_i\}_{i=1}^m$ are distinct in \cref{rs} in \cref{hyb2} is at least $1-\negl(\secp)$.
Therefore, we can assume  that all $\{r_i\}_{i=1}^m$ are distinct with a negligible loss in the adversary's winning probability.
If $r\notin\{r_i\}_{i=1}^m$, it is clear that $\cA$ cannot win the game of \cref{hyb2} except for a negligible probability.
The reason is that $\cA$ cannot find $\Sign(k,0\|r)$ or $\Sign(k,1\|r)$ except for a negligible probability due to the security of the digital signature scheme.
Therefore, we assume that $r$ is equal to one of the $\{r_i\}_{i=1}^m$.

Assume that, in the game of \cref{hyb2}, $\cC$ is replaced with $\cC'$ who is the same as $\cC$ except that
it measures the first qubit of $\ket{\psi_r}$ in the computational basis
before sending the states in \cref{send}.
Let $s\in\bit$ be the measurement result.
Then, for any QPT adversary $\cA$, the probability that $\cA$ wins
the game of \cref{hyb2}
is
negligible. The reason is that $\cA$ cannot find $\Sign(k,{s\oplus 1}\|r)$ 
except for a negligible probability due to the strong EUF-CMA security of the digital signature scheme.
From \cref{lem:BZ}, 
we therefore have
\begin{align}
   \Pr[(\Sign(k,0\|r),\Sign(k,1\|r))\gets\cA \mid \cC]&\le 2  
   \Pr[(\Sign(k,0\|r),\Sign(k,1\|r))\gets\cA \mid \cC']\label{ZB}\\
   &\le \negl(\secp), 
\end{align}
where the left-hand-side of \cref{ZB} is the probability that $\cA$ outputs
   $(\Sign(k,0\|r),\Sign(k,1\|r))$ with the challenger $\cC$,
   and the right-hand-side is that with the challenger $\cC'$.

==> security_old.tex <==
% !TEX root = main.tex
\section{Security}
In this section, we show IND-pkTA security of our construction. 
The outline of the proof is as follows.
The security game for the IND-pkTA security of our QPKE (Hybrid 0) is given in \cref{hyb0}.
We introduce two more hybrids, Hybrid 1 (\cref{hyb1}) and Hybrid 2 (\cref{hyb2}).
Hybrid 1 is the same as Hybrid 0 except that the challenger does not do the Hadamard-basis measurement
in the third step of $\Enc$ algorithm, and the challenger sends the adversary $r$ and the state over the registers
$(\regA,\regB,\regC)$.
Hybrid 2 is the same as Hybrid 1 except that the adversary outputs two bit strings $\alpha,\beta$ and
the adversary wins if $\alpha=\PRF_{k_0}(r)$ and $\beta=\PRF_{k_1}(r)$.

\ryo{I think we should write formal statements using the theorem environment, say, If PRF is pseudorandom and the signatures scheme is EUF-CMA, the scheme above satisfies IND-pkTA, something like that.}
\mor{I gave a formal theorem in the end of introduction. It's enough?}

Assume that the IND-pkTA security of our construction is broken by a QPT adversary
$\cA$. It means the QPT adversary $\cA$ wins Hybrid 0 with a non-negligible advantage.
Then, it is clear that there is another QPT adversary $\cA'$ that wins Hybrid 1 (\cref{hyb1}) 
with a non-negligible advantage. ($\cA'$ has only to do the Hadamard-basis measurement by itself.)
From the $\cA'$, we can construct a QPT adversary $\cA''$ that wins 
Hybrid 2 with a non-negligible probability 
by using the idea of \cite{HMY22} (\cref{sec:B}).
Finally, we show that
no QPT adversary can win the game of \cref{hyb2} except for a negligible probability (\cref{sec:Zhandry}).
We thus have the contradiction, and 
therefore our QPKE is IND-pkTA secure.

\protocol{Hybrid 0}
{Hybrid 0}
{hyb0}
{
\begin{enumerate}
    \item 
    The challenger $\cC$ chooses $k_0,k_1\gets\bit^\secp$.
    \item
    $\cC$ runs $(\mathsf{sigk},\vk)\gets\Gen(1^\secp)$.
    $\cC$ sends $\vk$ to $\cA$.
    \item
    \label{rs}
    $\cC$ chooses $r_1,...,r_m\gets\bit^u$.
    \item
    \label{send}
    $\cC$ sends $\{(r_i,\ket{\psi_0^{r_i}}+\ket{\psi_1^{r_i}})\}_{i=1}^m$
    to the adversary $\cA$, where
    \begin{align}
       \ket{\psi_0^{r_i}}&\coloneqq\ket{0}\otimes\ket{\PRF_{k_0}(r_i)}\otimes\ket{\sigma(r_i\|0\|\PRF_{k_0}(r_i))},\\
       \ket{\psi_1^{r_i}}&\coloneqq\ket{1}\otimes\ket{\PRF_{k_1}(r_i)}\otimes\ket{\sigma(r_i\|1\|\PRF_{k_1}(r_i))}. 
    \end{align}
    \item
    $\cA$ generates a quantum state over registers $\regA,\regB,\regC,\regD$. ($(\regA,\regB,\regC)$ corresponds to the quantum part of $\pk'$, and $\regD$ corresponds to $\st$.)
    $\cA$ sends a bit string $r$ and the registers $(\regA,\regB,\regC)$ to $\cC$.
    $\cA$ keeps the register $\regD$.
    \item
    \label{sign}
    $\cC$ coherently checks the signature in the state sent from $\cA$.
    If the result is $\bot$, it sends $\bot$ to $\cA$ and halts.
    If the result is $\top$, it goes to the next step. (If the probability that $\top$ is obtained is non-negligible,
    the state over the registers $(\regA,\regB,\regC,\regD)$ after the test is negligibly close to
    \begin{equation}
    c_0\ket{0}_\regA\ket{\PRF_{k_0}(r)}_\regB\ket{\Psi_0}_{\regC,\regD}    
    +c_1\ket{1}_\regA\ket{\PRF_{k_1}(r)}_\regB\ket{\Psi_1}_{\regC,\regD},   \label{why}
    \end{equation}
    where $c_0$ and $c_1$ are some complex coefficients such that $|c_0|^2+|c_1|^2=1$, 
and $\ket{\Psi_0}$ and $\ket{\Psi_1}$ are some normalized states.
For a proof, see \cref{app:why}.)
    \item
    $\cC$ applies $Z^b$ on the register $\regA$.
(If the state before the application of $Z^b$ is \cref{why}, it becomes
    \begin{equation} \label{eq:def_phi_b}
    \ket{\phi_b}\coloneqq c_0\ket{0}_\regA\ket{\PRF_{k_0}(r)}_\regB\ket{\Psi_0}_{\regC,\regD}    
    +(-1)^b c_1\ket{1}_\regA\ket{\PRF_{k_1}(r)}_\regB\ket{\Psi_1}_{\regC,\regD}
    \end{equation}
    after the application of $Z^b$.)
    \item
    $\cC$ measures all qubits in $(\regA,\regB,\regC)$ in the Hadamard basis to get the result $d$.
    $\cC$ sends $(r,d)$ to $\cA$.
    \item
    \label{last}
    $\cA$ outputs $b'$.
    If $b'=b$, $\cA$ wins.
\end{enumerate}
}


\protocol{Hybrid 1}
{Hybrid 1}
{hyb1}
{
\begin{itemize}
    \item[1.-7.]
    All the same as \cref{hyb0}.
    \item[8.]
    $\cC$ does not do the Hadamard-basis measurement,
    and $\cC$ sends $r$ and registers $(\regA,\regB,\regC)$ to $\cA$.
    \item[9.]
    The same as \cref{hyb0}.
\end{itemize}
}


\protocol{Hybrid 2}
{Hybrid 2}
{hyb2}
{
\begin{itemize}
    \item[1.-8.]
    All the same as \cref{hyb1}.
    \item[9.]
    $\cA$ outputs $(\alpha,\beta)$.
    If $\alpha=\PRF_{k_0}(r)$ and $\beta=\PRF_{k_1}(r)$, $\cA$ wins.
\end{itemize}
}







\input{why}



\subsection{Construction of $\cA''$}
\label{sec:B}

Assume that there exists a QPT adversary
$\cA'$ such that 
\begin{equation}
|\Pr[1\gets\cA'|b=0]-\Pr[1\gets\cA'|b=1]|=\Delta
\label{advantage}
\end{equation}
in the game of \cref{hyb1} with some non-negligible $\Delta$.
From the $\cA'$, we construct a QPT adversary $\cA''$ that wins the game of \cref{hyb2} with a non-negligible probability.

Let $\mathsf{Good}$ be the event that
$\cC$ gets $\top$ in \cref{sign} in the game of \cref{hyb1}.
If $\Pr[\mathsf{Good}]$ is negligible,
\cref{advantage} is not satisfied, because $\cA'$ receives only $\bot$ (which contains no information about $b$) except for a negligible probability.
Therefore, 
$\Pr[\mathsf{Good}]$ is non-negligible.

Assume that the event $\mathsf{Good}$ occurs.
Without loss of generality, we can assume that in \cref{last} of \cref{hyb1},
$\cA'$ applies a unitary $V$ on the state $\ket{\phi_b}$, and
measures the register $\regA$ in the computational basis to get $b'\in\bit$.
Then from \cref{advantage},
\begin{align}
V\ket{\phi_0}&=\sqrt{p}\ket{1}\ket{\nu_1}+\sqrt{1-p}\ket{0}\ket{\nu_0} \label{eq:V_phi_zero}\\    
V\ket{\phi_1}&=\sqrt{1-p+\Delta}\ket{0}\ket{\xi_0}+\sqrt{p-\Delta}\ket{1}\ket{\xi_1}    \label{eq:V_phi_one} 
\end{align}
for some real number $p$ and some normalized states $\ket{\nu_0},\ket{\nu_1},\ket{\xi_0},\ket{\xi_1}$.
(This is because any state can be written as $p\ket{1}\ket{\nu_1}+\sqrt{1-p}\ket{0}\ket{\nu_0}$
with some $p$ and normalized states $\ket{\nu_0},\ket{\nu_1}$, and due to \cref{advantage}, the coefficients
of $\ket{1}\ket{\xi_1}$ has to be $\sqrt{p-\Delta}$.)
If we define $W$ as
\begin{equation}
   W\coloneqq V^\dagger (Z\otimes I) V, 
\end{equation}
we have
\begin{align}
&   |
   c_0^*c_1\bra{0}\bra{\PRF_{k_0}(r)}\bra{\Psi_0}W\ket{1}\ket{\PRF_{k_1}(r)}\ket{\Psi_1}
   +c_0c_1^*\bra{1}\bra{\PRF_{k_1}(r)}\bra{\Psi_1}W\ket{0}\ket{\PRF_{k_0}(r)}\ket{\Psi_0}|\\
  &=\frac{1}{4} |
  (\bra{\phi_0}+\bra{\phi_1})W(\ket{\phi_0}-\ket{\phi_1})
  +(\bra{\phi_0}-\bra{\phi_1})W(\ket{\phi_0}+\ket{\phi_1})
  | \label{eq:rewrite}\\
  &=\frac{1}{2} |
  \bra{\phi_0}W\ket{\phi_0}
  -\bra{\phi_1}W\ket{\phi_1}
  |\\
   \begin{split}
   &=
  \frac{1}{2}\left|\left(\sqrt{p}\bra{1}\bra{\nu_1}+\sqrt{1-p}\bra{0}\bra{\nu_0}\right)
  \left(-\sqrt{p}\ket{1}\ket{\nu_1}+\sqrt{1-p}\ket{0}\ket{\nu_0}\right)\right.\\
  &\left.~~~-
    \left(\sqrt{1-p+\Delta}\bra{0}\bra{\xi_0}+\sqrt{p-\Delta}\bra{1}\bra{\xi_1}\right) 
  \left(\sqrt{1-p+\Delta}\ket{0}\ket{\xi_0}-\sqrt{p-\Delta}\ket{1}\ket{\xi_1}\right)\right|
  \end{split} \label{eq:expand}
  \\
  &=\frac{1}{2}\left|-p+(1-p)-(1-p+\Delta)+(p-\Delta)\right|\\
  & =\Delta 
\end{align}
where \Cref{eq:rewrite} follows from the definitions of $\ket{\phi_0}$ and $\ket{\phi_1}$ (\Cref{eq:def_phi_b}) and 
\Cref{eq:expand} follows from \Cref{eq:V_phi_zero,eq:V_phi_one} and the definition of $W$. 
From the triangle inequality and the facts that $|c_0|\le1$ and $|c_1|\le1$,
\begin{align}
&\Delta\le
   |c_1|\cdot|\bra{0}\bra{\PRF_{k_0}(r)}\bra{\Psi_0}W\ket{1}\ket{\PRF_{k_1}(r)}\ket{\Psi_1}|\\
   &+|c_0|\cdot|\bra{1}\bra{\PRF_{k_1}(r)}\bra{\Psi_1}W\ket{0}\ket{\PRF_{k_0}(r)}\ket{\Psi_0}|.
\end{align}
Then,
\begin{align}
\frac{\Delta}{2}\le
   |c_1|\cdot|\bra{0}\bra{\PRF_{k_0}(r)}\bra{\Psi_0}W\ket{1}\ket{\PRF_{k_1}(r)}\ket{\Psi_1}|
\end{align}
or
\begin{align}
&\frac{\Delta}{2}\le
  |c_0|\cdot|\bra{1}\bra{\PRF_{k_1}(r)}\bra{\Psi_1}W\ket{0}\ket{\PRF_{k_0}(r)}\ket{\Psi_0}|
\end{align}
holds.
Assume that the latter holds.
(The following proof can be easily modified even if the former holds.)
Then
\begin{align}
\frac{\Delta^2}{4}&\le
   |c_0|^2\cdot|\bra{1}\bra{\PRF_{k_1}(r)}\bra{\Psi_1}W\ket{0}\ket{\PRF_{k_0}(r)}\ket{\Psi_0}|^2\\
   &\le
   |c_0|^2\cdot\|(I\otimes\bra{\PRF_{k_1}(r)}\otimes I)W\ket{0}\ket{\PRF_{k_0}(r)}\ket{\Psi_0}\|^2.\label{delta}
\end{align}
With this $W$, we can construct the QPT adversary $\cA''$ that wins the game of \cref{hyb2} with a non-negligible probability as follows.
\begin{enumerate}
    \item 
    Simulate $\cA$ in steps 1.-8. of \cref{hyb2}. 
    If $\bot$ is sent from $\cC$, output $\bot$ and halt. 
    \item
    Measure the register $\regA$ of $\ket{\phi_b}$ in the computational basis. If the result is 1, output $\bot$ and halt.
    If the result is 0, measure the register $\regB$ of the post-measurement state in the computational basis to get the measurement result $\alpha$. 
    \item
    Apply $W$ on the post-measurement state 
    and measure the register $\regB$ in the computational basis to get the result $\beta$.
    Output $(\alpha,\beta)$.
\end{enumerate}
From the facts that $\Pr[\mathsf{Good}]$ is non-negligible,
$\alpha=\PRF_{k_0}(r)$ except for a negligible probability from \cref{app:why},
and 
\cref{delta},
the probability that $(\alpha,\beta)=(\PRF_{k_0}(r),\PRF_{k_1}(r))$ is
non-negligible.

\subsection{No QPT Adversary Can Win Hybrid 2 (\cref{hyb2})}
\label{sec:Zhandry}
Here we show that no QPT adversary can win Hybrid 2 (\cref{hyb2}) with a non-negligible probability.
First, note that the probability that all $\{r_i\}_{i=1}^m$ are distinct in \cref{rs} in \cref{hyb2} is at least $1-\negl(\secp)$.
Therefore, we can assume  that all $\{r_i\}_{i=1}^m$ are distinct with a negligible loss in the adversary's winning probability.
If $r\notin\{r_i\}_{i=1}^m$, it is clear that $\cA$ cannot win the game of \cref{hyb2} except for a negligible probability,
because due to the pseudorandamness of $\PRF$, $\PRF_{k_0}(r)$ and $\PRF_{k_1}(r)$ are
computationally indistinguishable from completely random bit strings.
Therefore, we assume that $r$ is equal to one of the $\{r_i\}_{i=1}^m$.

Assume that, in the game of \cref{hyb2}, $\cC$ is replaced with $\cC'$ who is the same as $\cC$ except that
it measures the first qubit of $\ket{\psi_0^r}+\ket{\psi_1^r}$ in the computational basis
before sending the states in \cref{send}.
Let $t\in\bit$ be the measurement result.
Then, for any QPT adversary $\cA$, the probability that $\cA$ wins
the game of \cref{hyb2}
is
negligible, because
$\PRF_{k_{s\oplus 1}}(r)$ is computationally indistinguishable from a complete random bit string to $\cA$, 
From \cref{lem:BZ}, 
we therefore have
\begin{align}
   \Pr[(\PRF_{k_0}(r),\PRF_{k_1}(r))\gets\cA|\cC]&\le 2  \Pr[(\PRF_{k_0}(r),\PRF_{k_1}(r))\gets\cA|\cC']\label{ZB}\\
   &\le \negl(\secp), 
\end{align}
where the left-hand-side of \cref{ZB} is the probability that $\cA$ outputs
   $(\PRF_{k_0}(r),\PRF_{k_1}(r))$ with the challenger $\cC$,
   and the right-hand-side is that with the challenger $\cC'$.
